Distributed Learning in Heterogeneous Environment: federated learning with adaptive aggregation and computation reduction

Although federated learning has achieved many breakthroughs recently, the heterogeneous nature of the learning environment greatly limits its performance and hinders its real-world applications. The heterogeneous data, time-varying wireless conditions and computing-limited devices are three main challenges, which often result in an unstable training process and degraded accuracy. Herein, we propose strategies to address these challenges. Targeting the heterogeneous data distribution, we propose a novel adaptive mixing aggregation (AMA) scheme that mixes the model updates from previous rounds with current rounds to avoid large model shifts and thus, maintain training stability. We further propose a novel staleness-based weighting scheme for the asynchronous model updates caused by the dynamic wireless environment. Lastly, we propose a novel CPU-friendly computation-reduction scheme based on transfer learning by sharing the feature extractor (FES) and letting the computing-limited devices update only the classifier. The simulation results show that the proposed framework outperforms existing state-of-the-art solutions and increases the test accuracy, and training stability by up to 2.38%, 93.10% respectively. Additionally, the proposed framework can tolerate communication delay of up to 15 rounds under a moderate delay environment without significant accuracy degradation.

==> Add.tex <==
\section{Experiments}
In this section, we conduct several experiments to analyse the performance of the proposed framework. Specifically, in section \ref{Sec5Sub1}, we demonstrate the performance improvement of the proposed method over the naive straggler-dropping scheme on different learning tasks. Then in section \ref{Sec5Sub2}, we compare the performance of the proposed method with \textit{FedProx}, and we show that our proposed method is more efficient.
\begin{figure*}[h]
    \centering
    \includegraphics[width=500]{Figs/Sec5/MNISTEandCIFAR10xperiments.pdf}
    \caption{Loss of the proposed framework and the naive straggler dropping scheme: The first row is the results for MNIST on the 5-layer CNN; the second row is the results for MNIST for the modified AlexNet; the third row is the results for CIFAR10 on the 5-layer CNN. Specifically, in each plot, 'DS' stands for 'Drop stragglers' while 'TL' stands for the  proposed framework. }
    \label{fig:Sec5Part1}
\end{figure*}
\subsection{Proposed Framework with Straggler-dropping}
\subsubsection{Experiment Setup}
To illustrate how the proposed framework improves the \textit{device heterogeneity} in the non-iid setting, we use the naive straggler-dropping scheme as the baseline. Specifically, we test the proposed method on two model structures. The first model is a simple 5-layer CNN, which consists of two convolutional layers and three fully connected layers. For the proposed framework, we fix the first two convolutional layers and only update the last-three layers, which are treated as the classifier, during the training session. The second model is the \textit{AlexNet}, consisting of 8 layers.  The first-5 layers are convolutional layers while the last 3 layers, which is the classifier,  are fully connected layers. During the training session, we fix the first-5 convolutional layers and only update the statistics of the classifier.  We modify the kernel size of the convolutional layers to accommodate the difference in the image size. 

We test the proposed method on two datasets. The first one is the MNIST handwritten digits, of which the sample size is $1*28*28$. The image is grey-scaled and thus has only one channel. For MNIST images, we set the communication round $B$ to be 200, the local epochs $E=10$ and the batch size ($bs$) as 20. The learning rate of the SGD optimiser $\eta=0.001$ and the momentum is set as 0.5. The number of selected clients in each round $m=10$. The second dataset is CIFAR10 \cite{cifar10}, which contains images of ships, birds, dogs, cats, etc.  The CIFAR10 images are colour-scaled and the dimension of the image is $3*32*32$. For CIFAR10, we set $B=500$, $E=5$, $bs=100$, $\eta=0.001$ and we increase the momentum of the SGD optimiser to 0.9. To impose the statistical heterogeneity, for both MNIST and CIAFR10, each client has access to images of 2 classes with 500 training samples and 100 testing samples. Regarding the device heterogeneity, before the training process starts, we randomly select $p\%$ of the clients to be stragglers and during the training session, before each communication round starts, $m=10$ clients are selected. Then during the local training stage, the stragglers are dropped in the baseline setting while in the proposed framework, the stragglers update the statistics of the classifier. 

\begin{figure*}[ht]
    \centering
    \includegraphics[width=500]{Figs/Sec5/Part2Experiments.pdf}
    \caption{Loss of the proposed framework and FedProx}
    \label{fig:Sec5Part2}
\end{figure*}

\subsubsection{Results}
The experiment results are shown in Fig. \ref{fig:Sec5Part1}. The first row and the second row show the results of the test loss for the MNIST digit recognition, comparing the proposed framework with the baseline on the 5-layer CNN and the AlexNet respectively.  When $p=0.25$ (the first column), the baseline (blue line) exhibits frequent but minor oscillations, whereas the proposed method (orange line) manages to reduce the magnitude of these peaks and smooth the loss curve for both models. It is worth noticing that the proposed method yields a lower loss for the 5-layer CNN throughout the learning process. As the level of device heterogeneity grows to $p=0.5$ and $p=0.75$, the baseline loss curves (orange line) swing even more violently because eliminating the straggler results in significant information loss. Nevertheless, the proposed method manages to regulate these peaks and provide a lower loss. 

The last row in Fig. \ref{fig:Sec5Part1} shows the loss on the CIFAR10 classification task on the 5-layer CNN. CIFAR10 is composed of three channels while the MNIST is grey-scaled, consisting of only one channel. Hence, the CIFAR10 classification task is more complex, and the loss curve dramatically oscillates in the non-iid setting. For $p=0.25$, the improvement of the proposed method (orange line) over the baseline (blue line) is not very distinct. This is probably because the impact of the non-iid data distribution, rather than the information loss caused by dropping stragglers, dominates the loss. However,  the proposed method provides a lower loss in general. As the device heterogeneity level increases, the baseline becomes even worse, with more frequent and larger oscillations. When $p=0.75$, the loss curve is hardly converging. In contrast, the proposed method reduces the oscillations significantly and obtains a much lower loss. In practical cases, a model with such performance may not be worth training but it can be seen that even in this situation, the proposed method can help improve the learning process. 

\textbf{Summary} After comparing the performance of the proposed method with the naive straggler-dropping scheme, we can see that the proposed method is generally effective in stabilising the learning process and achieving a lower loss.


\subsection{Proposed Framework with FedProx}
\subsubsection{Experiment Setup}
In this section, we compare the performance of the proposed method with \textit{FedProx}. As previously stated, \textit{FedProx} has two key ideas, the proximal term and the partial work. Here, we focus on investigating the device heterogeneity in the non-iid environment, therefore we neglect the proximal term for now and only compare the partial work with the proposed method. Specifically, to evaluate the performance of the partial work scheme, we set the local training epoch $E=1, 2, 3, 4$ respectively and count the number of local epochs required to achieve a comparable result with the proposed method. 

On the other hand, we consider the MNIST handwritten digits classification task on the 5-layer CNN, which has two convolutional layers and three fully-connected layers. For the proposed scheme, we only update the statistics of the classifier, that is the last three fully connected layers. Other experiment settings remain the same as in section \ref{Sec5Sub1},  $E=10, B=200, \eta=0.001, bs = 20, m=10 $ and the momentum of the SGD optimiser is 0.5. We vary the level of device heterogeneity from $p=0.25, 0.5$ to $p=0.75$. As in section \ref{Sec5Sub1}, each client has access to the samples of 2 digits, with 500 training samples and 100 testing samples in total. 

\subsubsection{Results}
The experiment results are shown in Fig. \ref{fig:Sec5Part2}. The notation PW=1  indicates that the straggler's local epoch is 1. When $p=0.75$, it shows that the proposed method (the blue solid line) yields a faster convergence and lower loss, compared with PW=1 and PW=2 (orange dash line). PW=3 reaches a comparable loss at the end but it converges slower and has larger oscillations. Nonetheless, PW=4 provides a similar convergence rate and comparable loss. It does, however, have larger oscillations than the proposed method. When $p=0.5$, the proposed method reaches a lower loss value than PW=1 while PW=2,3,4 reaches a comparable loss at the end but exhibits larger fluctuations. When $p=0.25$, the proposed framework and the partial work scheme have similar performances. As explained in \ref{Sec5Sub1}, when the number of stragglers is not large, the oscillations in loss curves are primarily caused by the statistical heterogeneity, leaving limited room for the proposed approach and partial-work scheme to improve.

\textbf{Summary} It is worth noticing that normally, updating a convolutional layer costs far more computation than a fully-connected layer. In our experiment setting, the first two convolutional layers consume approximately 2.7 times higher computation than the last three fully connected layers. Hence, when PW$\geq$3, the partial work scheme starts to consume more computation than the proposed framework under $E=10$. However, it shows that when $p=0.75$ and $p=0.5$, the proposed method has a smoother curve and slightly lower loss. PW=4 attains a similar performance to the proposed framework yet it consumes a lot more computation. Hence, it can be concluded that the proposed method is more efficient. 














==> Additional.tex <==
\section{Ease of Use}

\subsection{Maintaining the Integrity of the Specifications}

The IEEEtran class file is used to format your paper and style the text. All margins, 
column widths, line spaces, and text fonts are prescribed; please do not 
alter them. You may note peculiarities. For example, the head margin
measures proportionately more than is customary. This measurement 
and others are deliberate, using specifications that anticipate your paper 
as one part of the entire proceedings, and not as an independent document. 
Please do not revise any of the current designations.

\section{Prepare Your Paper Before Styling}
Before you begin to format your paper, first write and save the content as a 
separate text file. Complete all content and organizational editing before 
formatting. Please note sections \ref{AA}--\ref{SCM} below for more information on 
proofreading, spelling and grammar.

Keep your text and graphic files separate until after the text has been 
formatted and styled. Do not number text heads---{\LaTeX} will do that 
for you.

\subsection{Abbreviations and Acronyms}\label{AA}
Define abbreviations and acronyms the first time they are used in the text, 
even after they have been defined in the abstract. Abbreviations such as 
IEEE, SI, MKS, CGS, ac, dc, and rms do not have to be defined. Do not use 
abbreviations in the title or heads unless they are unavoidable.

\subsection{Units}
\begin{itemize}
\item Use either SI (MKS) or CGS as primary units. (SI units are encouraged.) English units may be used as secondary units (in parentheses). An exception would be the use of English units as identifiers in trade, such as ``3.5-inch disk drive''.
\item Avoid combining SI and CGS units, such as current in amperes and magnetic field in oersteds. This often leads to confusion because equations do not balance dimensionally. If you must use mixed units, clearly state the units for each quantity that you use in an equation.
\item Do not mix complete spellings and abbreviations of units: ``Wb/m\textsuperscript{2}'' or ``webers per square meter'', not ``webers/m\textsuperscript{2}''. Spell out units when they appear in text: ``. . . a few henries'', not ``. . . a few H''.
\item Use a zero before decimal points: ``0.25'', not ``.25''. Use ``cm\textsuperscript{3}'', not ``cc''.)
\end{itemize}

\subsection{Equations}
Number equations consecutively. To make your 
equations more compact, you may use the solidus (~/~), the exp function, or 
appropriate exponents. Italicize Roman symbols for quantities and variables, 
but not Greek symbols. Use a long dash rather than a hyphen for a minus 
sign. Punctuate equations with commas or periods when they are part of a 
sentence, as in:
\begin{equation}
a+b=\gamma\label{eq}
\end{equation}

Be sure that the 
symbols in your equation have been defined before or immediately following 
the equation. Use ``\eqref{eq}'', not ``Eq.~\eqref{eq}'' or ``equation \eqref{eq}'', except at 
the beginning of a sentence: ``Equation \eqref{eq} is . . .''

\subsection{\LaTeX-Specific Advice}

Please use ``soft'' (e.g., \verb|\eqref{Eq}|) cross references instead
of ``hard'' references (e.g., \verb|(1)|). That will make it possible
to combine sections, add equations, or change the order of figures or
citations without having to go through the file line by line.

Please don't use the \verb|{eqnarray}| equation environment. Use
\verb|{align}| or \verb|{IEEEeqnarray}| instead. The \verb|{eqnarray}|
environment leaves unsightly spaces around relation symbols.

Please note that the \verb|{subequations}| environment in {\LaTeX}
will increment the main equation counter even when there are no
equation numbers displayed. If you forget that, you might write an
article in which the equation numbers skip from (17) to (20), causing
the copy editors to wonder if you've discovered a new method of
counting.

{\BibTeX} does not work by magic. It doesn't get the bibliographic
data from thin air but from .bib files. If you use {\BibTeX} to produce a
bibliography you must send the .bib files. 

{\LaTeX} can't read your mind. If you assign the same label to a
subsubsection and a table, you might find that Table I has been cross
referenced as Table IV-B3. 

{\LaTeX} does not have precognitive abilities. If you put a
\verb|\label| command before the command that updates the counter it's
supposed to be using, the label will pick up the last counter to be
cross referenced instead. In particular, a \verb|\label| command
should not go before the caption of a figure or a table.

Do not use \verb|\nonumber| inside the \verb|{array}| environment. It
will not stop equation numbers inside \verb|{array}| (there won't be
any anyway) and it might stop a wanted equation number in the
surrounding equation.

\subsection{Some Common Mistakes}\label{SCM}
\begin{itemize}
\item The word ``data'' is plural, not singular.
\item The subscript for the permeability of vacuum $\mu_{0}$, and other common scientific constants, is zero with subscript formatting, not a lowercase letter ``o''.
\item In American English, commas, semicolons, periods, question and exclamation marks are located within quotation marks only when a complete thought or name is cited, such as a title or full quotation. When quotation marks are used, instead of a bold or italic typeface, to highlight a word or phrase, punctuation should appear outside of the quotation marks. A parenthetical phrase or statement at the end of a sentence is punctuated outside of the closing parenthesis (like this). (A parenthetical sentence is punctuated within the parentheses.)
\item A graph within a graph is an ``inset'', not an ``insert''. The word alternatively is preferred to the word ``alternately'' (unless you really mean something that alternates).
\item Do not use the word ``essentially'' to mean ``approximately'' or ``effectively''.
\item In your paper title, if the words ``that uses'' can accurately replace the word ``using'', capitalize the ``u''; if not, keep using lower-cased.
\item Be aware of the different meanings of the homophones ``affect'' and ``effect'', ``complement'' and ``compliment'', ``discreet'' and ``discrete'', ``principal'' and ``principle''.
\item Do not confuse ``imply'' and ``infer''.
\item The prefix ``non'' is not a word; it should be joined to the word it modifies, usually without a hyphen.
\item There is no period after the ``et'' in the Latin abbreviation ``et al.''.
\item The abbreviation ``i.e.'' means ``that is'', and the abbreviation ``e.g.'' means ``for example''.
\end{itemize}
An excellent style manual for science writers is \cite{b7}.

\subsection{Authors and Affiliations}
\textbf{The class file is designed for, but not limited to, six authors.} A 
minimum of one author is required for all conference articles. Author names 
should be listed starting from left to right and then moving down to the 
next line. This is the author sequence that will be used in future citations 
and by indexing services. Names should not be listed in columns nor group by 
affiliation. Please keep your affiliations as succinct as possible (for 
example, do not differentiate among departments of the same organization).

\subsection{Identify the Headings}
Headings, or heads, are organizational devices that guide the reader through 
your paper. There are two types: component heads and text heads.

Component heads identify the different components of your paper and are not 
topically subordinate to each other. Examples include Acknowledgments and 
References and, for these, the correct style to use is ``Heading 5''. Use 
``figure caption'' for your Figure captions, and ``table head'' for your 
table title. Run-in heads, such as ``Abstract'', will require you to apply a 
style (in this case, italic) in addition to the style provided by the drop 
down menu to differentiate the head from the text.

Text heads organize the topics on a relational, hierarchical basis. For 
example, the paper title is the primary text head because all subsequent 
material relates and elaborates on this one topic. If there are two or more 
sub-topics, the next level head (uppercase Roman numerals) should be used 
and, conversely, if there are not at least two sub-topics, then no subheads 
should be introduced.

\subsection{Figures and Tables}
\paragraph{Positioning Figures and Tables} Place figures and tables at the top and 
bottom of columns. Avoid placing them in the middle of columns. Large 
figures and tables may span across both columns. Figure captions should be 
below the figures; table heads should appear above the tables. Insert 
figures and tables after they are cited in the text. Use the abbreviation 
``Fig.~\ref{fig}'', even at the beginning of a sentence.

\begin{table}[htbp]
\caption{Table Type Styles}
\begin{center}
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Table}&\multicolumn{3}{|c|}{\textbf{Table Column Head}} \\
\cline{2-4} 
\textbf{Head} & \textbf{\textit{Table column subhead}}& \textbf{\textit{Subhead}}& \textbf{\textit{Subhead}} \\
\hline
copy& More table copy$^{\mathrm{a}}$& &  \\
\hline
\multicolumn{4}{l}{$^{\mathrm{a}}$Sample of a Table footnote.}
\end{tabular}
\label{tab1}
\end{center}
\end{table}

\begin{figure}[htbp]
\centerline{\includegraphics{fig1.png}}
\caption{Example of a figure caption.}
\label{fig}
\end{figure}

Figure Labels: Use 8 point Times New Roman for Figure labels. Use words 
rather than symbols or abbreviations when writing Figure axis labels to 
avoid confusing the reader. As an example, write the quantity 
``Magnetization'', or ``Magnetization, M'', not just ``M''. If including 
units in the label, present them within parentheses. Do not label axes only 
with units. In the example, write ``Magnetization (A/m)'' or ``Magnetization 
\{A[m(1)]\}'', not just ``A/m''. Do not label axes with a ratio of 
quantities and units. For example, write ``Temperature (K)'', not 
``Temperature/K''.

\section*{Acknowledgment}

The preferred spelling of the word ``acknowledgment'' in America is without 
an ``e'' after the ``g''. Avoid the stilted expression ``one of us (R. B. 
G.) thanks $\ldots$''. Instead, try ``R. B. G. thanks$\ldots$''. Put sponsor 
acknowledgments in the unnumbered footnote on the first page.

\section*{References}

Please number citations consecutively within brackets \cite{b1}. The 
sentence punctuation follows the bracket \cite{b2}. Refer simply to the reference 
number, as in \cite{b3}---do not use ``Ref. \cite{b3}'' or ``reference \cite{b3}'' except at 
the beginning of a sentence: ``Reference \cite{b3} was the first $\ldots$''

Number footnotes separately in superscripts. Place the actual footnote at 
the bottom of the column in which it was cited. Do not put footnotes in the 
abstract or reference list. Use letters for table footnotes.

Unless there are six authors or more give all authors' names; do not use 
``et al.''. Papers that have not been published, even if they have been 
submitted for publication, should be cited as ``unpublished'' \cite{b4}. Papers 
that have been accepted for publication should be cited as ``in press'' \cite{b5}. 
Capitalize only the first word in a paper title, except for proper nouns and 
element symbols.

For papers published in translation journals, please give the English 
citation first, followed by the original foreign-language citation \cite{b6}.

\begin{thebibliography}{00}
\bibitem{b1} G. Eason, B. Noble, and I. N. Sneddon, ``On certain integrals of Lipschitz-Hankel type involving products of Bessel functions,'' Phil. Trans. Roy. Soc. London, vol. A247, pp. 529--551, April 1955.
\bibitem{b2} J. Clerk Maxwell, A Treatise on Electricity and Magnetism, 3rd ed., vol. 2. Oxford: Clarendon, 1892, pp.68--73.
\bibitem{b3} I. S. Jacobs and C. P. Bean, ``Fine particles, thin films and exchange anisotropy,'' in Magnetism, vol. III, G. T. Rado and H. Suhl, Eds. New York: Academic, 1963, pp. 271--350.
\bibitem{b4} K. Elissa, ``Title of paper if known,'' unpublished.
\bibitem{b5} R. Nicole, ``Title of paper with only first word capitalized,'' J. Name Stand. Abbrev., in press.
\bibitem{b6} Y. Yorozu, M. Hirano, K. Oka, and Y. Tagawa, ``Electron spectroscopy studies on magneto-optical media and plastic substrate interface,'' IEEE Transl. J. Magn. Japan, vol. 2, pp. 740--741, August 1987 [Digests 9th Annual Conf. Magnetics Japan, p. 301, 1982].
\bibitem{b7} M. Young, The Technical Writer's Handbook. Mill Valley, CA: University Science, 1989.
\end{thebibliography}
\vspace{12pt}
\color{red}
IEEE conference templates contain guidance text for composing and formatting conference papers. Please ensure that all template text is removed from your conference paper prior to submission to the conference. Failure to remove the template text from your paper may result in your paper not being published.

==> Section2.tex <==
\section{Background and Related Work}\label{Sec2}
Heterogeneity in the mobile network is one of the key challenges in \textit{FL}. The traditional machine learning problem is solved in a central data processing platform while \textit{FL} has to deal with remote, highly distributed clients. Thus, it is hard to unify the computing standard for the clients. In general, the heterogeneity in the mobile network can be categorised into the following two aspects.

\subsection{Statistical Heterogeneity:}
The statistical heterogeneity refers to the non-iid distribution of the training samples. Machine learning algorithms need to learn from balanced datasets to obtain the best performance, while skewed data leads to performance degradation. Specifically, \cite{abs-1806-00582} shows that the deteriorated performance in the non-iid setting can be accounted for by the weight divergence. Let $\mathbf{w}_c^{T}$ denote the weights of the global model downloaded to each client at round $T$ before the local training starts, and $\mathbf{w}_k^{T}$, where $k$ is the client index, denote the weights of the updated local model after the local training. In iid setting, $\mathbf{w}_k^{T}$ for each client is closed to $\mathbf{w}_c^{T}$. In contrast, in the non-iid setting, $\mathbf{w}_k^{T}$ greatly diverges from the initial global model weights $\mathbf{w}_c^{T}$, and $\mathbf{w}_k^{T}$ for each client diverges from each other as well. \cite{abs-1806-00582} proves that this weight divergence is related to the distance between the local data distribution of each client.  As the skewness of the data distribution increases, the weight divergence becomes larger, leading to worse performance. Following this observation, \cite{abs-1806-00582} proposed to improve the model performance by sharing a balanced dataset. This public dataset reduces the distance between the data distribution of each client and thus reduces the divergence between the weights. Although experiments proved the effectiveness of \cite{abs-1806-00582}, it is unrealistic in practical cases since the such balanced datasets are hard to find. Moreover, sharing the data between the clients and the server violates the privacy-protecting rule of \textit{FL}.

On the other hand, \cite{ZhuHZ21} proposed \textit{FEDGEN} to perform the data augmentation based on knowledge distillation without directly sharing the dataset. Specifically, \textit{FEDGEN} learns a lightweight data generator which ensembles the data distribution knowledge of each client. This lightweight data generator is broadcast to each client to perform local data augmentation. Although no data is directly shared between the clients and the central server, still the local data distribution is observed by the central server. In sensitive applications, this can be considered privacy leakage and prohibitive.  In contrast, \cite{LuoCHZLF21} proposed to post-calibrate the classifier with virtual features. By examining the feature similarity between layers, \cite{LuoCHZLF21} proves that the classifier is most biased under the non-iid setting and proposes to calibrate the classifier after finishing the local training. Specifically, the model can be represented by a feature extractor and a classifier. Statistics of the feature extractor output for each client are gathered by the aggregation server and modelled with the Gaussian Mixture Model (GMM). The classifier is then calibrated with the virtual features sampled from the GMM model. 

Instead of modifying the data distribution, another way of mitigating the non-iid problem is to improve the model structure. \cite{abs-1912-00818} borrowed the idea from multitask learning and proposed \textit{FEDPER}, in which the local model combines the base layers and the personalised layers. Specifically, the base layers are shared between clients and trained with \textit{FedAvg} while the personalised layers are trained locally to cater for the impact of the statistical heterogeneity. Another example is \textit{MOON} \cite{LiHS21}. \textit{MOON} exploits the similarity between model representations and uses the global representation to de-bias the local representations. 


\subsection{Device Heterogeneity:}
In \textit{FL}, the resources of geographically distributed clients, such as the storage, the computation power and the communication bandwidth, are highly varied and this is referred to as the \textit{device heterogeneity}, also known as \textit{system heterogeneity} in some literature. Due to the disparity in computing and communication resources, some clients can not complete the training in time and such clients are called the \textit{stragglers}. The \textit{stragglers} are very common in practical \textit{FL} applications and can severely impede the learning process. As  mentioned above, naive \textit{FL} optimisation method, \textit{FedAvg} directly drops the \textit{stragglers}, leading to unstable and degraded model performance. Thus, sophisticated methods are needed to restore the model performance. 

The \textit{straggler} issue can be solved from different aspects. An intuitive way is to select participants with sufficient computation $\&$ communication resources. For example, \textit{FedMCCS} \cite{RahmanTMT21} determines whether a client is qualified for the training task with a linear regression model based on the CPU power, memory, and energy. In addition, \textit{FedMCCS} prioritises clients with rare class data to compensate for the statistical heterogeneity.  Similar works that select clients based on the computation or communication resources can be found in \cite{XuW21}, \cite{NishioY19}. In addition, \cite{abs-2010-01243} observed that training with clients having high local loss could accelerate the convergence. Following this observation, \cite{abs-2010-01243} proposed to select participants with higher local loss. \cite{abs-2010-01243} justified that a higher loss on a particular client means the model lacks the knowledge of it. Thus by learning more frequently from such clients, we can speed up the model convergence. Although participant selection avoids the straggler problem, it has several limitations. First, in scenarios that have a large number of stragglers, we may not have enough \textit{non-stragglers} to choose from. Secondly, it leads to the \textit{fairness} issue. Regardless of the selection criteria, the above methods all favour a specific group of clients, meaning the \textit{stragglers} have less chance of participating in the training process. Then it is unavoidable that these \textit{stragglers} would have a lower accuracy on the trained model, especially in non-iid settings. 
\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{Figs/Sec3/ProblemSetting.pdf}
    \caption{Problem Setting}
    \label{fig:Sec3ProblemSetting}
\end{figure}
On the other hand, asynchronous methods, such as \cite{abs-2102-06329}, which holds off the weights updates of the \textit{stragglers}, is another way of addressing the stragglers issue. However, it often requires one-to-one update routines and can be difficult to integrate with other \textit{FL} optimisation methods. Thus, it is impractical to implement such methods at a large scale. \cite{abs-2204-12703} proposed an ensemble \textit{FL} algorithm, \textit{Fed-ET}. targeting resource-constrained clients. The key idea is to train heterogeneous small models on the clients and then update the large central model at the server with these small models.  To cater for the statistical heterogeneity, \textit{Fed-ET} applies a weighted consensus distillation approach. Although the classification results on image and language tasks demonstrate the effectiveness of \textit{Fed-ET}, it requires specially designed small models for each client, which makes it impractical to implement at a large scale. 

% FedProx partial work and then compare my proposed method.
As mentioned above, \textit{FedProx} \cite{LiSZSTS20} not only mitigates the \textit{statistical heterogeneity} by adding a proximal term to the local loss function, it also addresses the \textit{straggler} problem by tolerating partial work. Specifically, in each communication round, the \textit{straggler} computes fewer rounds of local updates. \cite{LiSZSTS20} also provides the $\gamma_k^t-$\textit{inexact solution} to demonstrate the convergence results of this \textit{partial-work} scheme. On the other hand, in this work, we provide a more flexible way of reducing the computation load for the \textit{stragglers} by training only the classifier while stabilising the training performance. Compared to \textit{participant selection} methods \cite{RahmanTMT21} \cite{XuW21} \cite{NishioY19}, we include all the \textit{stragglers} in the training process, so the performance of the trained model on each client is more unified. Additionally, unlike the asynchronous methods \cite{abs-2102-06329}, and the ensemble transfer \textit{FL} \cite{abs-2204-12703}, our work requires only minor modifications for the training algorithm, and it can be easily integrated with other optimisation methods. Therefore, it is possible to be implemented on a large scale. 

























